Predicting Depth, Surface Normals and Semantic Labels with a Common Multi-Scale Convolutional Architecture

In this paper we address three different computer vision tasks using a single basic architecture: depth prediction, surface normal estimation, and semantic labeling. We use a multiscale convolutional network that is able to adapt easily to each task using only small modifications, regressing from the input image to the output map directly. Our method progressively refines predictions using a sequence of scales, and captures many image details without any superpixels or low-level segmentation. We achieve state-of-the-art performance on benchmarks for all three tasks.

==> normals_results_allgt.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{|cl||ccc|}
\hline
\multicolumn{5}{|c|}{\bf \small Surface Normal Estimation} \\
\hline
\hline
&&\multicolumn{3}{c|}{\bf Mean Angle Distance} \\
& & GT:\cite{fouhey13} & GT:\cite{ladicky14normals} & GT:\cite{Silberman12} \\
\hline
\hline
&3DP             & 34.2  &   35.3    &   37.7    \\
&Ladicky \aal    & 32.5  &   33.5    &   35.5    \\
&Fouhey \aal '14 & 35.1  &  --  &  -- \\
&Wang \aal       & 25.0  &  --  &  -- \\
&Ours            & 23.1  &   23.7    &   25.9    \\
&Ours (VGG)      & {\bf 20.5}  &   TODO    &   TODO    \\
\hline
\hline
\hline
& &\multicolumn{3}{c|}{\bf Median Angle Distance} \\
& & GT:\cite{fouhey13} & GT:\cite{ladicky14normals} & GT:\cite{Silberman12} \\
\hline
\hline
&3DP             & 30.0  &   31.2    &    34.1   \\
&Ladicky \aal    & 22.3  &   23.1    &    25.5   \\
&Fouhey \aal '14 & 19.2  &  --  &  -- \\
&Wang \aal       & 13.8  &  --  &  -- \\
&Ours            & 15.1  &  15.5  &  18.2   \\
&Ours (VGG)      & {\bf 13.2}  &  TODO  &  TODO   \\
\hline
\hline
\hline
\multicolumn{2}{|c||}{} 
&\multicolumn{3}{c|}{\bf \% Within $t^\circ$ Degrees} \\
\multicolumn{2}{|c||}{} 
& GT:\cite{fouhey13} & GT:\cite{ladicky14normals} & GT:\cite{Silberman12} \\
\hline
\hline
\multirow{4}{*}{$11.25^\circ$}
 & 3DP           & 18.5 &  16.4   &  14.0  \\
 & Ladicky \aal & 27.4 & 27.5  &  24.0    \\
 &Fouhey \aal '14 & 37.6  &  --  &  -- \\
 &Wang \aal       & {\bf 44.2}  &  --  &  -- \\
 & Ours          & 39.4  &  39.2  &  33.2   \\
 & Ours (VGG)    & 44.0  &  TODO  &  TODO   \\
\hline
\multirow{4}{*}{$22.5^\circ$}
 & 3DP           & 38.6 &  36.6   &  32.7  \\
 & Ladicky \aal & 50.2 & 49.0    &  45.6  \\
 &Fouhey \aal '14 & 53.3  &  --  &  -- \\
 &Wang \aal       & 63.2  &  --  &  -- \\
 & Ours          & 63.6  &  62.0  &  57.5   \\
 & Ours (VGG)    & {\bf 68.5}  &  TODO  &  TODO   \\
\hline
\multirow{4}{*}{$30^\circ$}
 & 3DP           & 50.0 &  48.2   &  44.1  \\
 & Ladicky \aal & 60.1 &  58.7   &  55.9  \\
 &Fouhey \aal '14 & 58.9  &  --  &  -- \\
 &Wang \aal       & 70.3  &  --  &  -- \\
 & Ours          & 72.7  &  71.1  &  67.7   \\
 & Ours (VGG)    & {\bf 77.2}  &  TODO  &  TODO   \\
\hline
\end{tabular}

\caption{Surface normals prediction measured against different types of ground truth acquisition.  Each column shows results for a different ground truth.}
\label{tab:normals}
\vspace{-4mm}
\end{table}







==> nyud_perclass_results.tex <==

\begin{table*}[h]
\centering


\begin{tabular}{cc}


{
\tiny
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|l|cccc|}
\hline
\multicolumn{5}{|c|}{\scriptsize {\bf 4-Class} (pixel acc.)} \\
\hline
\hline
& floor & struct & furntr & prop \\
\hline
Couprie \etal &   87.3 & 86.1 & 45.3 & 35.5 \\
Khan  \etal   &  87.1 &  88.2 & 54.7 & 32.6 \\
Stuckler \etal & 90.7 &  81.4  & 68.1  & 19.8 \\  
Mueller \etal &  {\bf 94.9} &  78.9  & 71.1  & 42.7 \\
Ours & 93.9 & {\bf 87.9} & {\bf 79.7} & {\bf 55.1} \\
\hline 
\end{tabular}
}



&    


{
\tiny
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|l|ccccccccccccc|}
\hline
\multicolumn{14}{|c|}{\scriptsize {\bf 13-Class} (pixel acc.)} \\
\hline
\hline
& bed & books & ceiling & chair & floor & furniture & objects & picture & sofa & table & tv & wall & window  \\
\hline
Couprie \etal & 30.3 & 31.7 & 33.2 & 44.4 & 68.0 & 28.5 & 10.9 & 38.5 & 25.8 & 18.0 & 18.8 & {\bf 89.4} & 37.8 \\
Wang \etal    & 47.6 & 45.0 & 68.1 & 23.5 & 84.1 & 16.7 & 12.4 & 26.4 & 39.1 & 35.4 & 32.4 & 65.9 & 52.2 \\
Hermans \etal & {\bf 68.4} & {\bf 45.4} & {\bf 83.4} & 41.9 & 91.5 & 37.1 & 8.6  & 35.8 & 28.5 & 27.7 & {\bf 38.4} & 71.8 & 46.1 \\
Khan \etal    & 38.1 & 13.7 & 62.6 & -    & 87.3 & -    & -    & -    & 29.8 & 10.2 & 6.0  & 86.1 & 15.9 \\
Ours          & 57.7 & 39.9 & 77.6 & {\bf 71.1} & {\bf 95.9} & {\bf 64.1} & {\bf 54.9} & {\bf 49.4} & {\bf 45.8} & {\bf 45.0} & 25.2 & 87.9 & {\bf 57.6}  \\
\hline
\end{tabular}
}

\end{tabular}



{
\tiny
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|l|cccccccccccccccccccc|}
\hline
\multicolumn{21}{|c|}{\scriptsize {\bf 40-Class} (Jaccard index)} \\
\hline
\hline

 & bag          
 & bathtub      
 & bed          
 & blinds       
 & book         
 & bookshelf    
 & box          
 & cabinet      
 & ceiling      
 & chair        
 & clothes      
 & counter      
 & curtain      
 & desk         
 & door         
 & dresser      
 & floor        
 & floor-mat    
 & fridge       
 & lamp         


\\

\hline

Gupta{\it \&al}'13

 & 0.65             
 & 33               
 & 55         
 & 44         
 & 4.4              
 & 20               
 & 4.8        
 & 48         
 & 59               
 & 40               
 & 6.9              
 & 47               
 & 34         
 & 10               
 & 8.3              
 & 22         
 & 81               
 & 22               
 & 15         
 & 6.8              

\\

Gupta{\it \&al}'14

 & 0.2              
 & {\bf 38.2}             
 & {\bf 65.0}             
 & 42.0             
 & 18.1             
 & 6.4              
 & 2.1              
 & 44.9             
 & 60.5             
 & {\bf 47.9}             
 & 4.7              
 & 51.3             
 & 29.1             
 & 11.3             
 & 20.3             
 & {\bf 34.8}             
 & 81.3             
 & 28.0             
 & 14.5             
 & {\bf 34.8}             


\\

Ours 

 &  1.5     
 &  29.1    
 &  51.9    
 &  43.9    
 &  16.6    
 &  31.5    
 &  4.5     
 &  45.0    
 &  {\bf 75.2}    
 &  46.0    
 &  12.9    
 &  53.4    
 &  35.4    
 &  11.3    
 &  17.6    
 &  26.3    
 &  83.3    
 &  27.4    
 &  15.7    
 &  33.6    

\\

Ours (VGG)

 &  {\bf 2.0}  
 &    37.3  
 &    58.6  
 &  {\bf 50.7}  
 &  {\bf 20.0}  
 &  {\bf 36.4}  
 &  {\bf 6.6}  
 &  {\bf 51.6}  
 &    66.0  
 &    47.5  
 &  {\bf 14.1}  
 &  {\bf 57.1}  
 &  {\bf 37.3}  
 &  {\bf 12.6}  
 &  {\bf 28.7}  
 &    24.3  
 &  {\bf 84.1}  
 &  {\bf 29.8}  
 &  {\bf 26.0}  
 &    31.2  



\\

\hline
\hline

 & mirror          
 & night-stand     
 & paper           
 & person          
 & picture         
 & pillow          
 & shelves         
 & showerctn       
 & sink            
 & sofa            
 & table           
 & toilet          
 & towel           
 & tv              
 & wall            
 & whitebd         
 & window          
 & other-furntr    
 & other-prop      
 & other-struct    
                   
\\






\hline

Gupta{\it \&al}'13

 & 19           
 & 20           
 & 1.9          
 & 16           
 & 40           
 & 28           
 & 5.1          
 & 18           
 & 26           
 & 44     
 & 30     
 & 50     
 & 14           
 & 9.3          
 & 68     
 & 37     
 & 33     
 & 2            
 & 22           
 & 6.9    

 \\

Gupta{\it \&al}'14

 & 16.4         
 & {\bf 27.2}         
 & 14.3         
 & 0.2          
 & 40.3         
 & {\bf 34.4}         
 & 3.5          
 & 4.2          
 & 37.5         
 & 47.9         
 & 29.9         
 & {\bf 55.1}         
 & 16.3         
 & 31.0         
 & 68.0         
 & 14.2         
 & 32.6         
 & 6.1          
 & 23.1         
 & 7.1          

 \\

Ours 


 &  {\bf 32.6}     
 &  24.2     
 &  20.3     
 &  27.5     
 &  45.0     
 &  31.0     
 &  8.9      
 &  {\bf 21.7}     
 &  39.4     
 &  40.4     
 &  32.0     
 &  44.8     
 &  14.8     
 &  32.3     
 &  68.2     
 &  6.6      
 &  33.0     
 &  6.8      
 &  {\bf 29.4}     
 &  11.7     

\\

Ours (VGG)


 &   23.3   
 &   24.7   
 & {\bf 21.2}   
 & {\bf 37.8}   
 & {\bf 48.5}   
 &   33.4   
 &  {\bf 9.1}   
 &   20.2   
 & {\bf 41.3}   
 & {\bf 49.1}   
 & {\bf 35.7}   
 &   44.0   
 & {\bf 20.0}   
 & {\bf 35.9}   
 & {\bf 71.1}   
 & {\bf 39.7}   
 & {\bf 37.4}   
 & {\bf 8.8}   
 &   28.7   
 & {\bf 13.1}   



\\

\hline
\end{tabular}
}


\label{tab:perclass}
\vspace{-3mm}
\end{table*}


